A Primer on Partial Wave Analysis

In the 90s of the last century high statistics experiments with fully equipped 4$\pi$ detectors have lead to a better insight in the spectrum of hadrons. In particular the finding of crypto-exotic and $J^{PC}$ exotic states tremendously improved the experimental situation in meson spectroscopy. All this was possible only with sophisticated analysis methods like the decomposition of measured phase-space distribution into partial waves and to express the partial waves in terms of complicated dynamical functions. This paper gives an introduction about the concepts and formalisms involved.

==> def_panda.tex <==
% def_panda.tex
%
\RequirePackage{xspace}
%
\def\ppbar{\ensuremath{\mbox{p}\overline{\mbox{p}}}\xspace}%
\def\pbarp{\ensuremath{\overline{\mbox{p}}\mbox{p}}\xspace}%
\def\pbarN{\ensuremath{\overline{\mbox{p}}\mbox{N}}\xspace}%
\def\pbard{\ensuremath{\overline{\mbox{p}}\mbox{d}}\xspace}%
\def\pbar{\ensuremath{\overline{\mbox{p}}}\xspace}%
\def\nbar{\ensuremath{\overline{\mbox{n}}}\xspace}%
\def\pbarn{\ensuremath{\overline{\mbox{p}}\mbox{n}}\xspace}%
\def\nbarn{\ensuremath{\overline{\mbox{n}}\mbox{n}}\xspace}%
%
\def\ccbar{\ensuremath{c\overline{c}}\xspace}%
\def\ccbarg{\ensuremath{c\overline{c}g}\xspace}%
\def\cqbar{\ensuremath{c\overline{q}}\xspace}%
\def\cbarq{\ensuremath{\overline{c}q}\xspace}%
\def\uubar{\ensuremath{u\overline{u}}\xspace}%
\def\ddbar{\ensuremath{d\overline{d}}\xspace}%
\def\ssbar{\ensuremath{s\overline{s}}\xspace}%
\def\bbbar{\ensuremath{b\overline{b}}\xspace}%
\def\bqbar{\ensuremath{b\overline{q}}\xspace}%
\def\bbarq{\ensuremath{\overline{b}q}\xspace}%
\def\qqbar{\ensuremath{q\overline{q}}\xspace}%
\def\qqbarg{\ensuremath{q\overline{q}g}\xspace}%
\def\QQbar{\ensuremath{Q\overline{Q}}\xspace}%
%
\def\ee{\ensuremath{e^+e^-}\xspace}%
\def\mumu{\ensuremath{\mu^+\mu^-}\xspace}%
%
\def\piz{\ensuremath{\pi^0}\xspace}%
\def\pip{\ensuremath{\pi^+}\xspace}%
\def\pim{\ensuremath{\pi^-}\xspace}%
\def\pipm{\ensuremath{\pi^\pm}\xspace}%
\def\pimp{\ensuremath{\pi^\mp}\xspace}%
%
\def\K{\ensuremath{K}\xspace}%
\def\Kp{\ensuremath{K^+}\xspace}%
\def\Km{\ensuremath{K^m}\xspace}%
\def\Kpm{\ensuremath{K^\pm}\xspace}%
\def\Kmp{\ensuremath{K^\mp}\xspace}%
\def\KKbar{\ensuremath{K\overline{K}}\xspace}%
\def\Kz{\ensuremath{K^0}\xspace}%
\def\Kzbar{\ensuremath{\overline{K}^0}\xspace}%
\def\KzKzbar{\ensuremath{K^0\overline{K^0}}\xspace}%
\def\Ks{\ensuremath{K_S^0}\xspace}%
\def\Kl{\ensuremath{K_L^0}\xspace}%
%
\def\etaprime{\ensuremath{\eta\prm}\xspace}%
\def\pione{\ensuremath{\pi_1}\xspace}%
%
\def\uquark{\ensuremath{u}\xspace}%
\def\dquark{\ensuremath{d}\xspace}%
\def\squark{\ensuremath{s}\xspace}%
\def\cquark{\ensuremath{c}\xspace}%
\def\bquark{\ensuremath{b}\xspace}%
\def\tquark{\ensuremath{t}\xspace}%
%
\def\D{\ensuremath{D}\xspace}%
\def\Dbar{\ensuremath{\overline{D}}\xspace}%
\def\DDbar{\ensuremath{D\overline{D}}\xspace}%
\def\DpDm{\ensuremath{D^+D^-}\xspace}%
\def\Dz{\ensuremath{D^0}\xspace}%
\def\Dzbar{\ensuremath{\overline{D}^0}\xspace}%
\def\DzDzbar{\ensuremath{D^0\overline{D}^0}\xspace}%
\def\Dx{\ensuremath{D^\ast}\xspace}%
\def\Dxbar{\ensuremath{\overline{D}^\ast}\xspace}%
\def\DxDxbar{\ensuremath{D^\ast\overline{D}^\ast}\xspace}%
\def\Dxz{\ensuremath{D^{\ast 0}}\xspace}%
\def\Dxzbar{\ensuremath{\overline{D}^{\ast 0}}\xspace}%
\def\DbarDxx{\ensuremath{D\overline{D}^{\ast\ast}}\xspace}%
%
\def\Ds{\ensuremath{D_s}\xspace}%
\def\Dspm{\ensuremath{D_s^\pm}\xspace}%
\def\Dsmp{\ensuremath{D_s^\mp}\xspace}%
\def\Dsx{\ensuremath{D_s^\ast}\xspace}%
\def\Dsxpm{\ensuremath{D_s^{\ast\pm}}\xspace}%
\def\Dsxmp{\ensuremath{D_s^{\ast\mp}}\xspace}%
\def\DsDsbar{\ensuremath{D_s\overline{D_s}}\xspace}%
\def\DspDsm{\ensuremath{D_s^+D_s^-}\xspace}%
\def\DsxDsxbar{\ensuremath{D_s^\ast\overline{D_s}^\ast}\xspace}%
\def\DsbarDsxx{\ensuremath{\overline{D_s}D_s^{\ast\ast}}\xspace}%
%
\def\jpsi{\ensuremath{J\!/\!\psi}\xspace}%
\def\psiprime{\ensuremath{\psi\prm}\xspace}%
\def\etac{\ensuremath{\eta_c}\xspace}%
\def\etacprime{\ensuremath{\eta^\prime_c}\xspace}%
\def\chicJ{\ensuremath{\chi_{cJ}}\xspace}%
\def\chiczero{\ensuremath{\chi_{c0}}\xspace}%
\def\chicone{\ensuremath{\chi_{c1}}\xspace}%
\def\chictwo{{\chi_{c2}}\xspace}%
\def\honec{\ensuremath{h_c}\xspace}%
%
\def\Cascade{\ensuremath{\Xi}\xspace}%
\def\Cascadebar{\ensuremath{\overline{\Xi}}\xspace}%
\def\LambdaLambdabar{\ensuremath{\Lambda\overline{\Lambda}}\xspace}%
\def\OmegaOmegabar{\ensuremath{\Omega\overline{\Omega}}\xspace}%
\def\SigmaSigmabar{\ensuremath{\Sigma\overline{\Sigma}}\xspace}%
\def\CascadeCascadebar{\ensuremath{\Xi\overline{\Xi}}\xspace}%
%
\def\degrees{{$^\circ$}\xspace}%
\def\percent{$\,$\%\xspace}%
%
\def\kev{{\mbox{keV}}\xspace}%
\def\kevcc{{\mbox{keV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mev{{\mbox{MeV}}\xspace}%
\def\mevc{{\mbox{MeV}\!/\!\mbox{\em c}}\xspace}%
\def\mevcc{{\mbox{MeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\mevccsq{{\mbox{MeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
\def\gev{{\mbox{GeV}}\xspace}%
\def\gevc{{\mbox{GeV}\!/\!\mbox{\em c}}\xspace}%
\def\gevcsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevcc{{\mbox{GeV}\!/\!\mbox{\em c$^2$}}\xspace}%
\def\gevccsq{{\mbox{GeV$^2$}\!/\!\mbox{\em c$^4$}}\xspace}%
%
\def\INST#1{{\sf\em #1}\xspace}%
\def\FNAL{\INST{FNAL}}%
\def\CERN{\INST{CERN}}%
\def\LEAR{\INST{LEAR}}%
\def\GSI{\INST{GSI}}%
\def\Panda{$\overline{\mbox{\sf P}}${\sf ANDA}\xspace}%
\def\HESR{\INST{HESR}}%
\def\Euro{{EUR}\xspace}%
%
\newcounter{auth}%
\setcounter{auth}{0}%
\def\authitem#1{\addtocounter{auth}{1}#1}%
\def\authitemi#1#2{\addtocounter{auth}{1}#2$^{#1}$}%
\newcounter{inst}%
\setcounter{inst}{0}%
\def\institem#1{\par \addtocounter{inst}{1}#1\\}%
\def\respitem#1{\institem{\underline{#1}}}%
\let\groupitem=\authitem
\def\lastitem{\ }%
%
\def\Journal#1#2#3#4{{\em #1}~{\bf #2} (#3) #4}%
\def\NPPS{{\em Nucl.~Phys.}~Proc.~Suppl.}%
\def\NCA{{\em Nuovo Cimento}}%
\def\NPA{{\em Nucl.~Phys.}~A}%
\def\NPB{{\em Nucl.~Phys.}~B}%
\def\PLA{{\em Phys.~Lett.}~A}%
\def\PLB{{\em Phys.~Lett.}~B}%
\def\PLD{{\em Phys.~Lett.}~D}%
\def\PL{{\em Phys.~Lett.}}%
\def\PRL{{\em Phys.~Rev.~Lett.}}%
\def\PREV{{\em Phys.~Rev.}}%
\def\PREP{{\em Phys.~Rep.}}%
\def\PRD{{\em Phys.~Rev.}~D}%
\def\PRC{{\em Phys.~Rev.}~C}%
\def\ZPC{{\em Z.~Phys.}~C}%
\def\ZPA{{\em Z.~Phys.}~A}%
\def\EPJA{{\em Eur.~J.~Phys.}~A}%
%
\def\bfg{\begin{figure}}%
\def\efg{\end{figure}}%
\def\bc{\begin{center}}%
\def\ec{\end{center}}%
\def\bi{\begin{itemize}}%
\def\ei{\end{itemize}}%
\def\be{\begin{equation}}%
\def\ee{\end{equation}}%
\def\bn{\begin{eqnarray}}%
\def\en{\end{eqnarray}}%
\def\ba#1{\left(\begin{array}{#1}}%
\def\ea{\end{array}\right)}%
\def\bef{\begin{equation}\fbox{$\displaystyle}%
\def\eef{$}\end{equation}}%
\def\bnf{\bef\ba{rcl}}%
\def\enf{\ea\eef}%
\def\refeq#1{eq.$\,$\ref{#1}}%
\def\refsec#1{sec.$\,$\ref{#1}}%
\def\reffig#1{fig.$\,$\ref{#1}}%
\def\reftbl#1{tbl.$\,$\ref{#1}}%
\def\ub{\underbrace}%
%
\def\vps{\hspace*{5mm}}%
\def\dsty{\displaystyle}%
% EOF: def_panda.tex


==> def_pwa.tex <==
% def_pwa.tex
%
\RequirePackage{xspace}
%
\def\mth#1{\ensuremath{#1}\xspace}%
%
\def\jpc{\mth{J^{P\!C}}}%
\def\ig{\mth{I^{G}}}%
\def\jpczeropm{\mth{\mbox{$0^{+-}$}}}%
\def\jpczeropp{\mth{\mbox{$0^{++}$}}}%
\def\jpczeromm{\mth{\mbox{$0^{--}$}}}%
\def\jpczeromp{\mth{\mbox{$0^{-+}$}}}%
\def\jpconepm{\mth{\mbox{$1^{+-}$}}}%
\def\jpconepp{\mth{\mbox{$1^{++}$}}}%
\def\jpconemm{\mth{\mbox{$1^{--}$}}}%
\def\jpconemp{\mth{\mbox{$1^{-+}$}}}%
\def\jpctwopm{\mth{\mbox{$2^{+-}$}}}%
\def\jpctwopp{\mth{\mbox{$2^{++}$}}}%
\def\jpctwomm{\mth{\mbox{$2^{--}$}}}%
\def\jpctwomp{\mth{\mbox{$2^{-+}$}}}%
%
\def\jpcscalar{\jpczeropp}%
\def\jpcvector{\jpconemm}%
\def\jpcaxialvector{\mth{\mbox{$1^{+\pm}$}}}%
\def\jpctensor{\jpctwopp}%
%
\def\Sif{\mth{S_{if}}}%
\def\Tif{\mth{T_{if}}}%
\def\Tdag{\mth{T^\dagger}}%
\def\LTif{\mth{\hat{T}_{if}}}%
\def\LT{\mth{\hat{T}}}%
\def\Kif{\mth{K_{if}}}%
\def\LKif{\mth{\hat{K}_{if}}}%
\def\LK{\mth{\hat{K}}}%
\def\Pi{\mth{P_{i}}}%
\def\LPi{\mth{\hat{P}_{i}}}%
\def\LP{\mth{\hat{P}}}%
\def\Br{\mth{B_{r}}}%
\def\Bri#1#2{\mth{B_{r,{#1}}^{#2}}}%
\def\Brqq#1{\mth{B_{r}^{#1}(q,q_{r})}}%
\def\massr{\mth{m_{r}}}%
\def\gammar{\mth{\Gamma_{r}}}%
\def\gammarz{\mth{\Gamma_{r}^0}}%
\def\MM{\mth{{\cal M}}}%
\def\Mif{\mth{\MM_{\rm if}}}%
\def\psit{\mth{\psi(t)}}%
\def\psitz{\mth{\psi(t=0)}}%
\def\ket#1{\mth{|{#1}\rangle}}%
\def\braket#1#2{\mth{\langle{#1}|{#2}\rangle}}%
\def\bra#1{\mth{\langle {#1}|}}%
\def\braf{\bra{f}}%
\def\brai{\bra{i}}%
\def\ketf{\ket{f}}%
\def\keti{\ket{i}}%
\def\DJmm{\mth{D^J_{m,m\prm}}}%
\def\dJmm{\mth{d^J_{m,m\prm}}}%
\def\DJmmOf#1#2{\mth{\DJmm(\theta,\varphi)}}%
\def\dJmmOf#1{\mth{\dJmm(\theta)}}%
\def\llab{\mth{\lone,\ltwo}}%
\def\llp{\mth{\lambda,\lambda\prm}}%
\def\als{\mth{\alpha_{ls}}}%
%
\def\Like{\mth{\cal L}}%
\def\logL{\mth{\ln\Like}}%
\def\chis{\mth{\chi^2}}%
%
\def\upup{\mth{\uparrow\uparrow}}%
\def\updown{\mth{\uparrow\downarrow}}%
\def\downup{\mth{\downarrow\uparrow}}%
\def\downdown{\mth{\downarrow\downarrow}}%
%
\def\FMab{\mth{m_{ab}}}%
\def\FMcd{\mth{m_{cd}}}%
\def\FMad{\mth{m_{ad}}}%
\def\FMac{\mth{m_{ac}}}%
\def\FMbc{\mth{m_{bc}}}%
\def\FMbd{\mth{m_{bd}}}%
\def\FMabS{\mth{m_{ab}^2}}%
\def\FMcdS{\mth{m_{cd}^2}}%
\def\FMadS{\mth{m_{ad}^2}}%
\def\FMacS{\mth{m_{ac}^2}}%
\def\FMbcS{\mth{m_{bc}^2}}%
\def\FMbdS{\mth{m_{bd}^2}}%
%
\def\TMab{\mth{m_{12}}}%
\def\TMac{\mth{m_{13}}}%
\def\TMbc{\mth{m_{23}}}%
\def\TMabS{\mth{m_{12}^2}}%
\def\TMacS{\mth{m_{13}^2}}%
\def\TMbcS{\mth{m_{23}^2}}%
%
\def\TSab{\mth{s_{12}}}%
\def\TSac{\mth{s_{13}}}%
\def\TSbc{\mth{s_{23}}}%
\def\TSz{\mth{s_0}}%
%
\def\pvec{\mth{\vec{p}}}%
\def\qvec{\mth{\vec{q}}}%
\def\rvec{\mth{\vec{r}}}%
\def\kvec{\mth{\vec{k}}}%
\def\xvec{\mth{\vec{x}}}%
\def\xveci{\mth{\vec{x}_i}}%
\def\xvecj{\mth{\vec{x}_j}}%
\def\pfr{\mth{\tilde{p}}}%
%
\def\dL{\mth{\partial L}}%
\def\dt#1{\mth{\frac{#1}{dt}}}%
\def\ddt{\mth{\dt{d}}}%
\def\xdot{\mth{\dot{x}}}%
\def\xidot{\mth{\dot{x_i}}}%
\def\xddot{\mth{\ddot{x}}}%
\def\xiddot{\mth{\ddot{x_i}}}%
\def\dx{\mth{\partial x}}%
\def\dxi{\mth{\partial{x_i}}}%
\def\dxdot{\mth{\partial\xdot}}%
\def\dxidot{\mth{\partial\xidot}}%
%
\def\prm{^{\prime}}%
\def\Nabla{\mth{\bigtriangledown}}%
\def\Laplace{\mth{\bigtriangleup}}%
\def\fpk{\mth{\frac{4\pi}{k}}}%
\def\dll{\mth{\delta_l}}%
\def\etl{\mth{\eta_l}}%
\def\suml{\mth{\sum_{l=0}^\infty}}%
\def\Exp#1{\mth{\dsty e^{\dsty #1}}}%
\def\oR{\mth{\omega_R}}%
\def\oZ{\mth{\omega_0}}%
\def\gamhalf{\mth{\frac{\Gamma}{2}}}%
\def\Det#1{\mth{\mbox{\em Det}\left[#1\right]}}%
\def\IM#1{\mth{\Im\left[#1\right]}}%
\def\RE#1{\mth{\Re\left[#1\right]}}%
\def\uln#1{\mth{U_l^n(#1)}}%
\def\Mathematica{{\tt Mathematica} $^{\mbox{\small TM}}$}%
\def\wht{\widehat}%
\def\inv{^{-1}}%
\def\half{{\frac{1}{2}}}%
\def\threehalf{{\frac{3}{2}}}%
\def\fivehalf{{\frac{5}{2}}}%
\def\Om{\Omega}%
\def\tht{\vartheta}%
\def\sth{\mth{\sin\tht}}%
\def\sths{\mth{\sin^2\tht}}%
\def\sthn#1{\mth{\sin^{#1}\tht}}%
\def\cth{\mth{\cos\tht}}%
\def\cths{\mth{\cos^2\tht}}%
\def\cthn#1{\mth{\cos^{#1}\tht}}%
\def\ph{\varphi}%
\def\AllJM{\mth{A_{\lone\ltwo}^{JM}}}%
\def\FllJ{\mth{F_{\lone\ltwo}^J}}%
\def\Tl{\mth{T_l}}%
\def\cnst{\mbox{const}}%
\def\lone{{\lambda_1}}%
\def\ltwo{{\lambda_2}}%
\def\lonetwo{{\lone\ltwo}}%
\def\dla{{\delta\lambda}}%
\def\CG#1#2#3{\mth{(#1\ #2|#3)}}%
\def\lamP{\lambda_{\mbox{\tiny p}}}
\def\lamN{\lambda_{\mbox{\tiny n}}}
%\def\spsi{height=4cm}%
%\def\spsii{height=2.5cm}%
%\def\spsi{scale=0.2}%
%\def\spsii{scale=0.5}%
%
% EOF: def_pwa.tex
